A multi-epoch spectral and photometric study to understand the nature of the interesting Be star candidate HD 249179

HD 249179, a B5 star with unclear classification as either a classical Be star or a high-mass X-ray binary (HMXB) system, is investigated using the first multi-epoch spectral and photometric analysis over 5.5 years (2017-2023). Optical spectroscopy from LAMOST, BeSS, and the Himalayan Chandra Telescope show large H-alpha variability (-17.6 to -3.2 angstrom, in six days, returning to -31.3 angstrom, in 2022) and the presence of Paschen and O I lines, confirming active circumstellar disc dynamics. H-alpha double peak profiles show weak V/R ratio variations 0.92--1.28 indicating one-armed density waves. TESS observations presents hybrid beta Cephei/slowly pulsating B-type variability with primary frequencies of 3.5 c/d and 1.5-1.6 c/d, and an outburst-like brightening with phase-dependent frequency evolution. Simultaneous anti-correlation between optical brightness and H$\alpha$ equivalent width suggest moderate disc inclination. Gaia DR3 CMD analysis rules out HD 249179 as a BeXRB but instead places it in the classical Be-star region. The BeppoSAX survey, despite previous X-ray cataloging, found no emission above the sensitivity limits. Our analysis shows that HD 249179 is most likely a classical Be star with variable circumstellar disc activity and hybrid pulsations, and that there is no strong evidence for an HMXB classification.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

